The 1/4-BPS building blocks of brane interactions

We study, from the perspective of supersymmetry and space-time Killing spinors, the local brane densities involved in 1/4-BPS intersecting brane systems. In particular, we classify the possible local brane structures that have maximal (16) supersymmetries in 1/4-BPS intersecting brane backgrounds. Applied to BPS black holes, this classification reveals the allowed local microstructure for pure microstates. We further use these structures with local 16 supersymmetries as building blocks to generalise to 1/8-BPS systems. Moreover, we give examples of 1/8-BPS black holes for which the local supersymmetries are compatible with the combination of different entropy-generating effects from brane interaction. Finally, applying our classification to BPS domain walls, we illustrate how our formalism may possibly describe the local picture of the Hanany-Witten effect.

==> Chapters/TikzDrawings/DualityMaps/DualityMapNonStandard.tex <==
\tikzsetnextfilename{DualityMapNonStandard}
\begin{tikzpicture}
    % Dp Dq scope
    \begin{scope}[node distance = 3cm and 4cm]
        % nodes Dp Dq (1)
        \node (D1D9) [IIB, on grid] {$\D{1} \parallel \D{9}$ (1)};
        \node (D2D8) [IIA, on grid, right = of D1D9] {$\D{2} \perp \D{8}$ (1)};
        \node (D3D7) [IIB, on grid, right = of D2D8] {$\D{3} \perp \D{7}$ (1)};
        \node (D4D6) [IIA, on grid, right = of D3D7] {$\D{4} \perp \D{6}$ (1)};
        \node (D5D5) [IIB, on grid, right = of D4D6] {$\D{5} \perp \D{5}$ (1)};
        % arrows between Dp Dq (1)
        % \draw [TDuality] (D1D9) to [bend left = 7] node[anchor=south] {$T_{\dashv}$} (D2D8);
        % \draw [TDuality] (D2D8) to [bend left = 7] node[anchor=north] {$T_{\vdash}$} (D1D9);
        % \draw [TDuality] (D2D8) to [bend left = 7] node[anchor=south] {$T_{\dashv}$} (D3D7);
        % \draw [TDuality] (D3D7) to [bend left = 7] node[anchor=north] {$T_{\vdash}$} (D2D8);
        % \draw [TDuality] (D3D7) to [bend left = 7] node[anchor=south] {$T_{\dashv}$} (D4D6);
        % \draw [TDuality] (D4D6) to [bend left = 7] node[anchor=north] {$T_{\vdash}$} (D3D7);
        % \draw [TDuality] (D4D6) to [bend left = 7] node[anchor=south] {$T_{\dashv}$} (D5D5);
        % \draw [TDuality] (D5D5) to [bend left = 7] node[anchor=north] {$T_{\vdash}$} (D4D6);
        \foreach \x in {1,...,4}
        {
            \pgfmathtruncatemacro{\y}{10 - \x}
            \pgfmathtruncatemacro{\u}{\x + 1}
            \pgfmathtruncatemacro{\v}{\y - 1}
            \draw [TDuality] ([yshift=.1cm]D\x D\y.east) to [bend left = 7] node[anchor=south] {$T_{\dashv}$} ([yshift=.1cm]D\u D\v.west);
            \draw [TDuality] ([yshift=-.1cm]D\u D\v.west) to [bend left = 7] node[anchor=north] {$T_{\vdash}$} ([yshift=-.1cm]D\x D\y.east);
        }
        
        % nodes Dp Dq (0)
        \node (D0D8) [IIA, on grid, below = of D1D9] {$\D{0} \parallel \D{8}$ (0)};
        \node (D1D7) [IIB, on grid, right = of D0D8] {$\D{1} \perp \D{7}$ (0)};
        \node (D2D6) [IIA, on grid, right = of D1D7] {$\D{2} \perp \D{6}$ (0)};
        \node (D3D5) [IIB, on grid, right = of D2D6] {$\D{3} \perp \D{5}$ (0)};
        \node (D4D4) [IIA, on grid, right = of D3D5] {$\D{4} \perp \D{4}$ (0)};
        % arrows between Dp Dq (0)
        % \draw [TDuality] (D0D8) to [bend left = 7] node[anchor=south] {$T_{\dashv}$} (D1D7);
        % \draw [TDuality] (D1D7) to [bend left = 7] node[anchor=north] {$T_{\vdash}$} (D0D8);
        % \draw [TDuality] (D1D7) to [bend left = 7] node[anchor=south] {$T_{\dashv}$} (D2D6);
        % \draw [TDuality] (D2D6) to [bend left = 7] node[anchor=north] {$T_{\vdash}$} (D1D7);
        % \draw [TDuality] (D2D6) to [bend left = 7] node[anchor=south] {$T_{\dashv}$} (D3D5);
        % \draw [TDuality] (D3D5) to [bend left = 7] node[anchor=north] {$T_{\vdash}$} (D2D6);
        % \draw [TDuality] (D3D5) to [bend left = 7] node[anchor=south] {$T_{\dashv}$} (D4D4);
        % \draw [TDuality] (D4D4) to [bend left = 7] node[anchor=north] {$T_{\vdash}$} (D3D5);
        \foreach \x in {0,...,3}
        {
            \pgfmathtruncatemacro{\y}{8 - \x}
            \pgfmathtruncatemacro{\u}{\x + 1}
            \pgfmathtruncatemacro{\v}{\y - 1}
            \draw [TDuality] ([yshift=.1cm]D\x D\y.east) to [bend left = 7] node[anchor=south] {$T_{\dashv}$} ([yshift=.1cm]D\u D\v.west);
            \draw [TDuality] ([yshift=-.1cm]D\u D\v.west) to [bend left = 7] node[anchor=north] {$T_{\vdash}$} ([yshift=-.1cm]D\x D\y.east);
        }

        % arrows between Dp Dq (1) and Dp Dq (0)
        \foreach \x in {1,...,5}
        {
            \pgfmathtruncatemacro{\y}{10 - \x}
            \pgfmathtruncatemacro{\u}{\x - 1}
            \pgfmathtruncatemacro{\v}{\y - 1}
            \draw [TDuality] ([xshift=.1cm]D\x D\y.south) to [bend left = 7] node[anchor=west] {$T_{\parallel}$} ([xshift=.1cm]D\u D\v.north);
            \draw [TDuality] ([xshift=-.1cm]D\u D\v.north) to [bend left = 7] node[anchor=east] {$T_{\perp}$} ([xshift=-.1cm]D\x D\y.south);
        }
    \end{scope}

    
    % Dp KKM/NS5/KKM* scope
    \begin{scope}[node distance = 3cm and 5cm, yshift = -7cm]
        % nodes Dp KKM 
        \node (D2KKM) [IIA, on grid] {$\D{2} \perp \KKM$ (0)};
        \node (D3KKM) [IIB, on grid, below = of D2KKM] {$\D{3} \perp \KKM$ (1)};
        \node (D4KKM) [IIA, on grid, below = of D3KKM] {$\D{4} \perp \KKM$ (2)};
        \node (D5KKM) [IIB, on grid, below = of D4KKM] {$\D{5} \perp \KKM$ (3)};
        \node (D6KKM) [IIA, on grid, below = of D5KKM] {$\D{6} \perp \KKM$ (4)};
        \node (D7KKM) [IIB, on grid, below = of D6KKM] {$\D{7} \parallel \KKM$ (5)};
        % arrows between Dp KKM and Dp+1 KKM 
        \foreach \x in {2,...,6}
        {
            \pgfmathtruncatemacro{\y}{\x + 1}
            \draw [TDuality] ([xshift=.1cm]D\x KKM.south) to [bend left = 7] node[anchor=west] {$T_{\dashv}$} ([xshift=.1cm]D\y KKM.north);
            \draw [TDuality] ([xshift=-.1cm]D\y KKM.north) to [bend left = 7] node[anchor=east] {$T_{\parallel}$} ([xshift=-.1cm]D\x KKM.south);
        }

        % nodes Dp NS5
        \node (D3NS5) [IIB, on grid, right = of D2KKM] {$\D{3} \perp \NS$ (0)};
        \node (D4NS5) [IIA, on grid, below = of D3NS5] {$\D{4} \perp \NS$ (1)};
        \node (D5NS5) [IIB, on grid, below = of D4NS5] {$\D{5} \perp \NS$ (2)};
        \node (D6NS5) [IIA, on grid, below = of D5NS5] {$\D{6} \perp \NS$ (3)};
        \node (D7NS5) [IIB, on grid, below = of D6NS5] {$\D{7} \perp \NS$ (4)};
        \node (D8NS5) [IIA, on grid, below = of D7NS5] {$\D{8} \parallel \NS$ (5)};
        % arrows between Dp NS5 and Dp+1 NS5
        \foreach \x in {3,...,7}
        {
            \pgfmathtruncatemacro{\y}{\x + 1}
            \draw [TDuality] ([xshift=.1cm]D\x NS5.south) to [bend left = 7] node[anchor=west] {$T_{\dashv}$} ([xshift=.1cm]D\y NS5.north);
            \draw [TDuality] ([xshift=-.1cm]D\y NS5.north) to [bend left = 7] node[anchor=east] {$T_{\parallel}$} ([xshift=-.1cm]D\x NS5.south);
        }
        % arrows between Dp KKM and Dp+1 NS5
        \foreach \x in {2,...,7}
        {
            \pgfmathtruncatemacro{\y}{\x + 1}
            \draw [TDuality] ([yshift=.1cm]D\x KKM.east) to [bend left = 7] node[anchor=south] {$T_{\dashv*}$} ([yshift=.1cm]D\y NS5.west);
            \draw [TDuality] ([yshift=-.1cm]D\y NS5.west) to [bend left = 7] node[anchor=north] {$T_{\vdash}$} ([yshift=-.1cm]D\x KKM.east);
        }
        
        
        % nodes Dp KKM *
        \node (D4KKM*) [IIA, on grid, right = of D3NS5] {$\D{4} \perp \KKM$ (0)*};
        \node (D5KKM*) [IIB, on grid, below = of D4KKM*] {$\D{5} \perp \KKM$ (1)*};
        \node (D6KKM*) [IIA, on grid, below = of D5KKM*] {$\D{6} \perp \KKM$ (2)*};
        \node (D7KKM*) [IIB, on grid, below = of D6KKM*] {$\D{7} \perp \KKM$ (3)*};
        \node (D8KKM*) [IIA, on grid, below = of D7KKM*] {$\D{8} \perp \KKM$ (4)*};
        \node (D9KKM*) [IIB, on grid, below = of D8KKM*] {$\D{9} \parallel \KKM$ (5)*};
        % arrows between Dp KKM and Dp+1 KKM
        \foreach \x in {4,...,8}
        {
            \pgfmathtruncatemacro{\y}{\x + 1}
            \draw [TDuality] ([xshift=.1cm]D\x KKM*.south) to [bend left = 7] node[anchor=west] {$T_{\dashv}$} ([xshift=.1cm]D\y KKM*.north);
            \draw [TDuality] ([xshift=-.1cm]D\y KKM*.north) to [bend left = 7] node[anchor=east] {$T_{\parallel}$} ([xshift=-.1cm]D\x KKM*.south);
        }
        % arrows between Dp KKM and Dp+1 NS5
        \foreach \x in {3,...,8}
        {
            \pgfmathtruncatemacro{\y}{\x + 1}
            \draw [TDuality] ([yshift=.1cm]D\x NS5.east) to [bend left = 7] node[anchor=south] {$T_{\perp}$} ([yshift=.1cm]D\y KKM*.west);
            \draw [TDuality] ([yshift=-.1cm]D\y KKM*.west) to [bend left = 7] node[anchor=north] {$T_{\dashv*}$} ([yshift=-.1cm]D\x NS5.east);
        }
    \end{scope}


    % NS5/KKM (1) scope
    \begin{scope}[node distance = 3cm and 5cm, xshift=16cm, yshift = -7cm]
        % nodes P/F1 NS5/KKM
        \node (NS5NS5) [IIAB, on grid] {$\NS \perp \NS$ (1)};
        \node (NS5KKM*) [IIAB, on grid, below = of NS5NS5] {$\NS \perp \KKM$ (1)*};
        \node (KKMKKM**) [IIAB, on grid, below = of NS5KKM*] {$\KKM \perp \KKM$ (1)**};
        % arrows between P Dp and P Dp+1
        \draw [TDuality] ([xshift=.1cm]NS5NS5.south) to [bend left = 7] node[anchor=west] {$T_{\dashv}$} ([xshift=.1cm]NS5KKM*.north);
        \draw [TDuality] ([xshift=-.1cm]NS5KKM*.north) to [bend left = 7] node[anchor=east] {$T_{\parallel*}$} ([xshift=-.1cm]NS5NS5.south);
        \draw [TDuality] ([xshift=.1cm]NS5KKM*.south) to [bend left = 7] node[anchor=west] {$T_{\vdash}$} ([xshift=.1cm]KKMKKM**.north);
        \draw [TDuality] ([xshift=-.1cm]KKMKKM**.north) to [bend left = 7] node[anchor=east] {$T_{*\parallel}$} ([xshift=-.1cm]NS5KKM*.south);
        \draw [TDuality] ([xshift=-.7cm]KKMKKM**.north) to [bend left = 30] node[anchor=east] {$T_{\parallel*,\leftrightarrow}$} ([xshift=-.7cm]NS5KKM*.south);
    \end{scope}


    % NS5/KKM (3) scope
    \begin{scope}[node distance = 3cm and 5cm, xshift=16cm, yshift = -16cm]
        % nodes P/F1 NS5/KKM
        \node (NS5KKM) [IIAB, on grid,] {$\NS \perp \KKM$ (3)};
        \node (KKMKKM*) [IIAB, on grid, below = of NS5KKM] {$\KKM \perp \KKM$ (3)*};
        % arrows between P Dp and P Dp+1
        \draw [TDuality] (NS5KKM) to [out=20, in=340, loop] node[anchor=south west] {$T_{\dashv*,\leftrightarrow}$} ();
        \draw [TDuality] ([xshift=.1cm]NS5KKM.south) to [bend left = 7] node[anchor=west] {$T_{\dashv}$} ([xshift=.1cm]KKMKKM*.north);
        \draw [TDuality] ([xshift=-.1cm]KKMKKM*.north) to [bend left = 7] node[anchor=east] {$T_{*\parallel}$} ([xshift=-.1cm]NS5KKM.south);
    \end{scope}

    
    % S duality arrows
    \begin{scope}
        \draw [SDuality] (D5KKM*) to [bend left = 20] node[anchor=south] {$S$} (NS5KKM*);
        \draw [SDuality] (D3NS5) to [bend left = 20] node[anchor=north west] {$S$} (D3D5);
        \draw [SDuality] (D5D5.east) to [bend left = 20] node[anchor=west] {$S$} (NS5NS5.east);
        \draw [SDuality] (D5KKM) to [bend left = 15] node[anchor=south] {$S$} (NS5KKM);
        
        \draw [SDuality] (D3KKM) to [loop left] node[anchor=east] {$S$} ();
        \draw [SDuality] (D5NS5) to [out=30, in=50, loop] node[anchor=south west] {$S_{\leftrightarrow}$} ();
        \draw [SDuality] (KKMKKM**) to [loop below] node[anchor=north] {$S$} ();
    \end{scope}
\end{tikzpicture}


==> Chapters/TikzDrawings/GeometryHananyWitten/Hanany-Witten_effect.tex <==
\tikzsetnextfilename{Hanany-Witten_effect}
	\begin{adjustbox}{max totalsize={\textwidth}{\textheight},center}
		\begin{tikzpicture}
			\begin{scope}[shift={(0,0)}]

				% D8 region
				\draw [ black, line width=1.5 ] (-9,-4) -- (-11,-6) -- (-11,4) --(-9,6) -- cycle;
				\node[align = center, centered, fill=white] at (-10, -6.5) {\Huge D8};
				%
				% F1
				\draw [ blue, line width=1.5] (-10, 0) --(1.5,0);
				\node[align = center, centered] at (-4.5, -1) {\Huge F1};
				%
				% D0
				\filldraw[black] (1.5,0) circle (4pt);
				\node[align = center, centered] at (1.5, -1) {\Huge D0};
			\end{scope}
			%
		\end{tikzpicture}
	\end{adjustbox}

==> Chapters/TikzDrawings/GeometryHananyWitten/Hanany-Witten_microscopic.tex <==
\tikzsetnextfilename{Hanany-Witten_microscopic}
	\begin{adjustbox}{max totalsize={\textwidth}{\textheight},center}
		\begin{tikzpicture}
			\begin{scope}[shift={(0,0)}]
			    % Cap
				\draw[black,line width=1.5] (0, 1.5) arc (90:-90:1.5);
				%\draw [gray, thick,dashed](0.0,0) circle [x radius=0.3, y radius=1.5];
				\draw[gray, thick,dashed] (0,1.5) arc (90:-90: 0.3 and 1.5 );
				\draw[black, thick,dashed] (0,-1.5) arc (-90:-270: 0.3 and 1.5 );
				%
				% Throat
				\draw [ black, line width=1.5] (0, 1.5) --(-6,1.5);
				\draw [ black, line width=1.5] (0, -1.5) --(-6,-1.5);
				%
				\draw[gray, thick,dashed] (-6,1.5) arc (90:-90: 0.3 and 1.5 );
				\draw[black, thick,dashed] (-6,-1.5) arc (-90:-270: 0.3 and 1.5 );
				%
				%
				% S^7
				\node[] at (-6, 2.5) {\Huge $S^7$};
				%
				%
				% BIon spike
				\draw[black, line width=1.5] (-6,-1.5) to[out=180, in=90] (-10, -4);
				\draw[black, line width=1.5] (-6,1.5) to[out=180, in=-90] (-10, 4);
				%
				% D8 region
				\draw [ black, line width=1.5 ] (-9,-4) -- (-11,-6) -- (-11,4) --(-9,6);
				\draw [ black, line width=1.5 ] (-9,6) -- (-9,2.25);
				\draw [ black, line width=1.5 ] (-9,-4) -- (-9,-2.25);
				%
				% Names of the regions
				\node[align = center, centered] at (0.375, -6) {\LARGE D0-F1\\\LARGE region};
				\node[align = center, centered, fill=white] at (-9, -6) {\LARGE D8-F1\\ \LARGE region };
				% 
				%
			\end{scope}
			%
		\end{tikzpicture}
	\end{adjustbox}

==> Chapters/TikzDrawings/LuninMathurPath.tex <==
\tikzsetnextfilename{Lunin-Mathur-Path}
\begin{tikzpicture}[node distance = 3cm and 6cm]

    \node (PF1) [IIB, on grid, rectangle split, rectangle split parts=2, draw, align=center] 
    {$\W[y] \parallel \F[y]$ (1) \nodepart{second} 
        $\W[1] \parallel \F[1]$ \\
        $\W[2] \parallel \F[2]$ \\
        $\W[4] \parallel \F[4]$ \\
        $\W[9] \parallel \F[9]$ 
    };


    
    \node (PNS5) [IIB, on grid, right = of PF1, yshift = 2cm, rectangle split, rectangle split parts=2, draw, align=center] 
    {$\W[y] \parallel \NS[y1234]$ (1) \nodepart{second} 
        $\D[1]{1} \perp \D[234]{3}$ \\
        $\D[2]{1} \perp \D[134]{3}$ \\
        $\D[4]{1} \perp \D[123]{3}$ \\
        $\W[9] \parallel \NS[12349]$ 
    };
    \node (placeholder) [on grid, right = of PNS5]{};
    \node (D1D5) [IIB, on grid, right = of placeholder, rectangle split, rectangle split parts=2, draw, align=center] 
    {$\D[y]{1} \parallel \D[y1234]{5}$ (1) \nodepart{second} 
        $\F[y] \parallel \NS[y1234]$ \\
        $\D[y12]{3} \perp \D[y34]{3}$ \\
        $\D[y14]{3} \perp \D[y23]{3}$ \\
        $\W[9] \parallel \KKM[12349;y]$ 
    };

    \draw [TDuality,->] ([yshift=0.5cm]PF1.east) to node[anchor=south, sloped] {$S, T_{1,2,3,4},S$} (PNS5.west);
    \draw [TDuality,->] (PNS5.east) to node[anchor=south] {$T_{y,1},S$} (D1D5.west);



    \node (F1D1) [IIB, on grid, right = of PF1, yshift = -2cm, rectangle split, rectangle split parts=2, draw, align=center] 
    {$\F[y] \perp \D[1]{1}$ (0) \nodepart{second} 
        $\F[1] \perp \D[y]{1}$ \\
        $\W[2] \parallel \D[y12]{3}$ \\
        $\W[4] \parallel \D[y14]{3}$ \\
        $\W[9] \parallel \D[y19]{3}$ 
    };
    \node (D1D3) [IIB, on grid, right = of F1D1, rectangle split, rectangle split parts=2, draw, align=center] 
    {$\D[y]{1} \perp \D[123]{3}$ (0) \nodepart{second} 
        $\D[1]{1} \perp \D[y23]{3}$ \\
        $\D[2]{1} \perp \D[y13]{3}$ \\
        $\W[4] \parallel \NS[y1234]$ \\
        $\W[9] \parallel \NS[y1239]$ 
    };
    \node (D1D52) [IIB, on grid, right = of D1D3, rectangle split, rectangle split parts=2, draw, align=center] 
    {$\D[y]{1} \parallel \D[y1234]{5}$ (1) \nodepart{second} 
        $\D[y14]{3} \perp \D[y23]{3}$ \\
        $\D[y24]{3} \perp \D[y13]{3}$ \\
        $\F[y] \parallel \NS[y1234]$ \\
        $\W[9] \parallel \KKM[12349;y]$ 
    };

    \draw [TDuality,->] ([yshift=-0.5cm]PF1.east) to node[anchor=south, sloped] {$S, T_{y,1}$} (F1D1.west);
    \draw [TDuality,->] (F1D1.east) to node[anchor=south] {$T_{2,3}, S$} (D1D3.west);
    % \draw [TDuality,->] (D1D3.east) to node[anchor=south] {$T_{y,4}$} (D1D52.west);
    \draw [TDuality,->] (D1D3.east) to node[anchor=south] {$T_{y,4}, (y \leftrightarrow 4)$} (D1D52.west);

    \draw [SDuality] (F1D1) to [loop below] node[anchor=north] {$S_{\leftrightarrow}$} ();
    
\end{tikzpicture}
